A General Theory of Additive State Space Abstractions

Informally, a set of abstractions of a state space S is additive if the distance between any two states in S is always greater than or equal to the sum of the corresponding distances in the abstract spaces. The first known additive abstractions, called disjoint pattern databases, were experimentally demonstrated to produce state of the art performance on certain state spaces. However, previous applications were restricted to state spaces with special properties, which precludes disjoint pattern databases from being defined for several commonly used testbeds, such as Rubiks Cube, TopSpin and the Pancake puzzle. In this paper we give a general definition of additive abstractions that can be applied to any state space and prove that heuristics based on additive abstractions are consistent as well as admissible. We use this new definition to create additive abstractions for these testbeds and show experimentally that well chosen additive abstractions can reduce search time substantially for the (18,4)-TopSpin puzzle and by three orders of magnitude over state of the art methods for the 17-Pancake puzzle. We also derive a way of testing if the heuristic value returned by additive abstractions is provably too low and show that the use of this test can reduce search time for the 15-puzzle and TopSpin by roughly a factor of two.

==> fanSTRIPSrep.tex <==

\subsection{Simple examples for using the STRIPS model}
Section \ref{fixreference} and \ref{pancake-costsplitting} have shown two methods of defining additive abstractions for the pancake puzzle. Now assume that the operators of the pancake puzzle are presented by the STRIPS model, we show how to define additive abstractions for this model. In the examples shown in Figure \ref{fig-pancake-locationbased} and Figure \ref{fig-pancake-costsplitting}, R2 is to reverse the order of the first two tiles and R4 is to reverse the total four tiles. The grounded operators (R2 and R4) are defined by three set of atoms: the precondition list (P), add list (A) and delete list (D). Atom (at location-num tile-num) means that tile tile-number is located in the location location-num. For example, atom (at 1 3) indicates that tile 3 is located in the the first location. The first abstraction is achieved by  ``dropping'' all atoms in the form of (at - 2) or (at - 4); the second abstraction ``drops'' all atoms in the form of (at - 1) or (at - 3). For the sake of simplicity, we always define the residual cost of each individual edge $R_i(\pi_i)=C(\pi)-C_i(\pi_i)$. Then it would be not difficult to verify that the abstractions satisfy the three conditions and the resulting heuristics generated from two abstractions are additive.

\subsubsection{Location-based Costs}
Now we assign primary costs using location-based method. An abstract state transition has a primary cost of 1 if the operator adding list A involves (at 1 -) (e.g. (at 1 1) or (at 1 4)); otherwise the primary cost is zero. In another word, if an abstract state transition changes the tile in the first location of the permutation, the primary cost is one; otherwise, it is zero cost. The middle and right parts of Figure \ref{fig-pancake-locationbased} describe the primary cost of each individual abstract state transition. Solid arrows denote abstract state transitions with the primary cost of one, and dashed arrows denote abstract state transitions with the primary cost of zero.
\begin{figure}[!ht]
\centerline{
\includegraphics[height=4.6cm]{pancake-original.pdf} 
\includegraphics[height=4.6cm]{pancake-abs1-locationbased.pdf}
\includegraphics[height=4.6cm]{pancake-abs2-locationbased.pdf}
}
\caption{A simple example to define additive abstractions using location-based costs. An abstract state transition has a primary cost of 1 if the operator adding list A involves (at 1 -); otherwise the primary cost is zero. (Left: original state transitions. Middle: state transitions in the first abstract state space. Right: state transitions in the second abstract state space.)}
\label{fig-pancake-locationbased}
\end{figure}

\subsubsection{Cost-Splitting}
\begin{figure}[!ht]
\centerline{
\includegraphics[height=4.6cm]{pancake-original.pdf} 
\includegraphics[height=4.6cm]{pancake-abs1-costsplitting.pdf}
\includegraphics[height=4.6cm]{pancake-abs2-costsplitting.pdf}
}
\caption{A simple example to define additive abstractions using cost-splitting. Each abstract state transition has a primary cost of $1/2$. (Left: original state transitions. Middle: state transitions in the first abstract state space. Right: state transitions in the second abstract state space.)}
\label{fig-pancake-costsplitting}
\end{figure}
There are several ways to apply the method cost-splitting. We just present a simple example. As shown in Figure \ref{fig-pancake-costsplitting}, there are two atoms in the add list of the gounded operator R2 in original state space, and in each abstract space, there are only one atom in the add list of R2. Therefore, in the abstract space we assign the primary cost of R2=$\frac{1}{2}$. In the same manner, the primary cost of R4 is defined to be $\frac{2}{4}$, i.e. $\frac{1}{2}$.

\subsection{Logistics Domain}
Figure \ref{fig-logistics} and Figure \ref{fig-logistics-groundedop} present an instance in Logistics Domain.
\begin{figure}[!ht]
\centerline{
\includegraphics[height=5cm]{logistics.pdf} 
\includegraphics[height=5cm]{logistics-goal.pdf}
}
\caption{A simple example of the Logistics Problem. The left part is an arrangement satisfying the initial state description and the right part is one arrangement corresponding to the goal description.}
\label{fig-logistics}
\end{figure}
In the following subsections, we show that besides Edelkamp's mehod, we can create two additive abstractions for {\bf Logistics} domain by at least three other methods. The key point of all the following methods is to satisfy the requirements in our definition for additive abstraction. For the sake of simplicity, we assume that these two abstractions are homomorphisms of the original state space and we always define the residual cost of each individual edge $R_i(\pi_i)=C(\pi)-C_i(\pi_i)$.
\subsubsection{Method I: Partitioning the edges by directions}
{\bf Left edges} (i.e. move the object close to office2) are defined by the following grounded operators.

drive (truck1 office1 office2)

P=$\{$(at truck1 office1)$\}$,

A=$\{$(at truck1 office2)$\}$, and

D=$\{$(at truck1 office1)$\}$.

load (package1 truck1 office1)

P=$\{$(at truck1 office1) (in package1 office1)$\}$,

A=$\{$(in package1 truck1) $\}$, and

D=$\{$(in package1 office1)$\}$.

load (package2 truck1 office1)

P=$\{$(at truck1 office1) (in package2 office1)$\}$,

A=$\{$(in package2 truck1) $\}$, and

D=$\{$(in package2 office1)$\}$.

unload (package2 truck1 office2)

P=$\{$(at truck1 office2) (in package2 truck1)$\}$,

A=$\{$(in package2 office2) $\}$, and

D=$\{$(in package2 truck1)$\}$.

unload (package1 truck1 office2)

P=$\{$(at truck1 office2) (in package1 truck1)$\}$,

A=$\{$(in package1 office2) $\}$, and

D=$\{$(in package1 truck1)$\}$.

{\bf Right edges} (i.e. move the object close to office1) are defined by the following grounded operators.

drive (truck1 office2 office1)

P=$\{$(at truck1 office2)$\}$,

A=$\{$(at truck1 office1)$\}$, and

D=$\{$(at truck1 office2)$\}$.

load (package1 truck1 office2)

P=$\{$(at truck1 office2) (in package1 office2)$\}$,

A=$\{$(in package1 truck1) $\}$, and

D=$\{$(in package1 office2)$\}$.

load (package2 truck1 office2)

P=$\{$(at truck1 office2) (in package2 office2)$\}$, and

D=$\{$(in package2 office2)$\}$.

unload (package1 truck1 office1)

P=$\{$(at truck1 office1) (in package1 truck1)$\}$,

A=$\{$(in package1 office1)$\}$, and

D=$\{$(in package1 truck1)$\}$.

unload (package2 truck1 office1)

P=$\{$(at truck1 office1) (in package2 truck1)$\}$,

A=$\{$(in package2 office1)$\}$, and

D=$\{$(in package2 truck1)$\}$.

In the first abstraction, the primary cost of each {\bf left} edge is assigned to be the same as the edge cost in the original state space and the primary cost of each right edge is zero.

In the second abstraction, the primary cost of each {\bf right} edge is assigned to be the same as the edge cost in the original state space and the primary cost of each left edge is zero.  

By this method, the first abstraction is only concerned with the left edge costs and the second only counts the right edge costs. Thus the resulting heuristics generated by these two abstractions are additive.

\subsubsection{Method II--Partitioning the edges by operator's add list}
We define an {\bf office1} edge if its operator's add list includes state variable ''office1''. For example, unload (package2 truck1 office1) is an {\bf office1} edge because its add list A=$\{$(in package2 office1)$\}$.

We define a {\bf non-office1} edge if its operator's add list does not include state variable ''office1''. For example, load (package2 truck1 office2) is a {\bf non-office1} edge because its add list A=$\{$(in package2 truck1)$\}$.

In the first abstraction, the primary cost of each {\bf office1} edge is assigned to be the same as the edge cost in the original state space and the primary cost of other individual edge is zero.

In the second abstraction, the primary cost of each {\bf non-office1} edge is assigned to be the same as the edge cost in the original state space and the primary cost of other individual edge is zero.  

By this method, the first abstraction is only concerned with the {\bf office1} edge  costs and the second only count the {\bf non-office1} edge costs. Thus the resulting heuristics generated by these two abstractions are additive.

\subsubsection{Method III--Cost Splitting}
Cost Splitting is a generalized method that we can apply it to any state space. To construct two additive abstractions, we can assign the primary cost to be the half of its preimage edge cost in the original state space,i.e.,$C_i(\pi_i)=C(\pi)/2$. 

In this way, we satisfy the requirement for additive abstractions.
\subsubsection{Discussion}
In the above examples for Method I and Method II, the primary cost $C_i$ is assigned to be the cost of its preimage in the original space, or zero cost. There are numerous other methods to assign the value the primary cost, by which the three conditions are satisfied. However, how to assign abstracted edge costs for better balancing between abstractions and how to select effective additive abstraction-based heuristics are still open research topics.

In practice, we always assign values to the primary cost according to the operators/actions properties, such as the direction of the action, the target of the action, the precondition of the action, or the effect of the action, etc. In addition, to identify infeasibility, the residual cost $R_i$ is always defined to be its maximum permitted value.

Now we have shown how to define additive abstractions for a pathfinding problem domain. By Lemma 3.4 and Lemma 3.5, $\hadd$ is admissible as well as consistent. These methods can be easily generalized to any other pathfinding problem domains. 



==> guidline.tex <==

\section{How to apply our methodology to a new domain}
\label{sec-guideline}
\MEMO{What to do with this section ? Rob is inclined to delete it rather
than trying to fix it.}
This section provides a detailed description to give an idea of what to do in order to use our general methodology to a new domain. First we present a guideline to apply this general method. Then we translate the pancake puzzle using the STRIPS model and show how to define additive abstractions for this model. In the end, we show that besides Edelkamp's method, we can create two additive abstractions for the Logistics domain by at least three other methods.

\subsection{A Guideline}
Given multiple abstractions of a new domain, we can do the following to define additive abstractions.
\begin{enumerate}
\item Assign a value to the primary cost of each edge in the abstraction to satisfy the condition  that  $\forall \gpr \in \gpairs, \gcost(\gpr) \ge \sum_{i=1}^k \abcost{i}(\abpr{i})$. In this step, we can assign the values according to any structural properties of the domain, such as the property of the operators and the property of the state which the edge is incident from or to.
\item Since we require that $\forall \gpr \in \gpairs, \gcost(\gpr) \ge \abcost{i}(\abpr{i}) + \abresid{i}(\abpr{i})$, in order to identify infeasibility the residual cost $R_i$ is always defined to be its maximum permitted value. For example, $\abresid{i}(\abpr{i})= \gcost(\gpr)-\abcost{i}(\abpr{i})$. 
\item Given a state $t$ and a goal state $g$, we compute $C_i^*(t_i,g_i)$, the minimum primary cost of an abstract path from $t_i$ to $g_i$. As defined in Section 3.3, the additive-abstraction-based heuristic value $\haddtg=\sum_{i=1}^k \abminc{i}(\abst{i},\abgoal{i})$.
\item If $\haddtg < \hmaxtg $ does not hold for a large fraction of the state space $\gstates$, we have generated effective additive abstractions; otherwise go back to step 1 to assign new values to the primary costs.   

\end{enumerate}

In short, we can create additive abstractions for any domain if the definitions of the primary cost $\abcost{i}$ and the residual cost $\abresid{i}$ satisfy the following three conditions.
\begin{eqnarray}
\forall (u,v) \in \gpairs, (\abmap{i}(u),\abmap{i}(v)) \in \gpairs{i} & & \label{COSTCOND}
\end{eqnarray}
\begin{eqnarray}
\forall \gpr \in \gpairs, \gcost(\gpr) \ge \sum_{i=1}^k \abcost{i}(\abpr{i})
& & \label{COSTCOND2}
\end{eqnarray}
\begin{eqnarray}
\forall \gpr \in \gpairs, \gcost(\gpr) \ge \abcost{i}(\abpr{i}) + \abresid{i}(\abpr{i}) & & \label{COSTCOND3}
\end{eqnarray}
Then the additive heuristic for state $t$ given a set of abstractions
%% mappings $\mapset = \{ \abmap{1}, \dots, \abmap{k} \}$
and goal state g is formally defined to be

\begin{center}
$\haddtg=\sum_{i=1}^k \abminc{i}(\abst{i},\abgoal{i})$
\end{center}



==> haslum01.tex <==

\begin{eqnarray*}
h^m(t) & = & \left\{ \begin{array}{ll}
	0, & t \subseteq start\\
	\min_{(s,t)\in\Pi} C(s,t) + h^m(s), & |t| \le m\\
	\max_{s\subset t \; \mbox{ and} \; |s| \le m} h^m(s), & |t| > m
	\end{array}
	\right.
\end{eqnarray*}



==> logistics-example.tex <==

%%
To illustrate this method consider the simplified
%% definition of the
Logistics domain
%% with the start and goal states depicted graphically
%% in Figure \ref{fig-logistics}
defined by the
grounded operators shown in
Figure \ref{fig-logistics-groundedop}.
There are three different types of objects---``$package$"
(the packages to be transported), ``$truck$" and ``$location$"---and
three operators:
``$unload$" (move the object in the vehicle to the location),
``$load$" (move the object at the location into the vehicle), and
``$drive$" (move the vehicle from one location to another location).
One possible abstraction is to delete from the state descriptions
and grounded operator definitions any atoms that do not refer to ``package2".
Figure \ref{fig-abstractlogistics} shows the resulting abstract state space.

\begin{figure}[!h!t]
%\includegraphics[height=7.4cm]{logistics-groundedop-load.pdf}
%\includegraphics[height=7.4cm]{logistics-groundedop-unload.pdf}
\centerline{
\includegraphics[height=7cm]{logistics-groundedop-Left.pdf}
\includegraphics[height=7cm]{logistics-groundedop-Right.pdf}
}
%\includegraphics[height=3.7cm,trim= 0 5cm 0 0]{logistics-groundedop-drive.pdf}

\caption{Grounded operators of the Logistics domain. In the description for each action, P, A and D represent the precondition list, add list and delete list, respectively.}
\label{fig-logistics-groundedop}
\end{figure}

\begin{figure}[!ht]
\centerline{
\includegraphics[height=5cm]{logistics-abstraction.pdf}
}
\caption{An abstract state space for the Logistics problem based on keeping only the atoms that mention ``package2". Self-loops have been omitted.}
\label{fig-abstractlogistics}
\end{figure}



==> newApplicationsIntroOLD.tex <==

\section{New Applications of Additive Abstractions}
\label{applications}

This section and the next section report
the results of applying the general definition
of additive abstraction given in the previous section to three
benchmark state spaces: TopSpin, Rubik's Cube,
and the Pancake puzzle.\footnote{A few additional experimental results
may be found in \cite{additiveTheory07}.}
For these state spaces
a state $t$ is represented by a vector of $m$ state variables
all defined over the same domain of possible values $D$, {\em i.e.},
$t=(t(0),..., t(m-1))$, where $t(j) \in D$ is the value assigned
to the $j^{th}$ state variable in state $t$.
There is one variable for each physical location in the puzzle,
and the value of $t(j)$ indicates which ``tile" is in location $j$ in state $t$.
State space abstractions are defined by abstracting the domain $D$.
In particular,
domain abstraction $\abmap{i}$ will leave specific domain values unchanged
(the ``distinguished tiles" according to $\abmap{i}$)
and map all the rest to the same special value, ``don't care".
The abstract state corresponding to $t$ according to $\abmap{i}$ is
$t_i$=$(t_i(0),...,t_i(m-1))$ with $t_i(j) = \abmap{i}(t(j))$.
As in previous research with these state spaces all edges (state transitions)
have a cost of one and a set of abstractions is defined by partitioning
the tiles.\footnote{The theory developed in the previous section
does not require the distinguished tiles in different abstractions
to be mutually exclusive; it allows a tile to be distinguished in any
number of abstract spaces provided abstract costs are defined appropriately.}

Where we differ from previous research is in how we define the cost of
an abstract state transition $\abcost{i}(\abpr{i})$.\footnote{In all our
experiments we define $R_i(\abpr{i}) = 1 - \abcost{i}(\abpr{i})$,
its maximum permitted value when edges cost 1.}
We consider two methods of defining costs,
called ``cost-splitting" and ``location-based".
These are general in the sense that they can be applied to any state space
of the type being considered,
{\em i.e.}, whose state transitions can be described as moving
tiles among locations.

In cost-splitting, a state transition $\pi$ that moves $b^{\pi}$ tiles has its
cost, $C(\pi)$, split among the abstractions $\abmap{1}, \dots ,\abmap{k}$
in proportion to the number of distinguished tiles it moves
for each abstraction, {\em i.e.}:

\[
\abcost{i}(\abpr{i})= \frac{b^{\pi}_i*C(\pi)}{b^{\pi}}
\]

\noindent
if $\pi$ moves $b^{\pi}$ tiles and $b^{\pi}_i$ of them
are distinguished according to $\abmap{i}$.\footnote{Because $\abpr{i}$ might
correspond to several edges in the the original space, each with a different
cost or moving a different set of tiles, the technically correct
definition is:
\[
\abcost{i}(\abpr{i})= \min_{\mbox{\small $\{\pi \setdelim \abmap{i}(\pi)=\abpr{i}\}$}}\{\frac{b^{\pi}_i*C(\pi)}{b^{\pi}}\}
\]
\label{minfootnote} } If each tile is distinguished in at most one
abstraction ({\em e.g.}\ if the abstractions are defined by partitioning
the tiles) cost-splitting produces additive abstractions, {\em
i.e.},
$\gcost(\gpr) \ge \sum_{i=1}^k
\abcost{i}(\abpr{i})$ for all $\gpr \in \gpairs$.
For example, in Rubik's Cube each operator moves eight
cubies,\footnote{A ``cubie" is one of the twenty little moveable
cubes that make up the $3 \times 3 \times 3$ Rubik's cube. This
example assumes that a cubie plays the role of a ``tile".}
%%, which is true in some, but not all, encodings of the puzzle
%% \cite{maxingAIJ06}.}
four corner cubies and four edge cubies.
Hence $b^{\pi}=8$ for all state transitions $\pi$.
If a particular state transition moves three cubies that are
distinguished according to abstraction $\psi_i$, the corresponding
abstract state transition, $\abpr{i}$, would cost $\frac{3}{8}$.



In location-based cost definitions, a reference location
$loc_{\pi}$ is associated with state transition $\pi$ and $\pi$'s
full cost $C(\pi)$ is assigned to abstract state transition
$\abpr{i}$ if $\abpr{i}$ changes the tile in location $loc_{\pi}$
(it may change any number of tiles in non-reference locations) and
the tile that $\pi$ moves into $loc_{\pi}$ is a distinguished tile
according to $\abmap{i}$, {\em i.e.}:\footnote{Analogous to
footnote \ref{minfootnote}, the technically correct definition has
$\min_{\mbox{\small $\{\pi \setdelim \abmap{i}(\pi)=\abpr{i}\}$}}\{C(\pi)\}$
instead of $C(\pi)$.}

\[
\abcost{i}(\abpr{i})= \left\{
  \begin{array}{ll}
    C(\pi), & \mbox{if $\pi_i = (t^1_i,t^2_i)$, $t^1_i(loc^{\pi}) \ne t^2_i(loc^{\pi})$, and}\\
                            & \mbox{$t^2_i(loc^{\pi})$ is a distinguished tile according to $\abmap{i}$.}
\\
    0, & \mbox{otherwise.}
  \end{array} \right.
\]

Instead of focusing on the tile that moves into $loc_{\pi}$, one can
equally well define location-based costs on the tile that moves out
of $loc_{\pi}$. In either case, if each tile is distinguished in at
most one abstraction location-based costs produce additive
abstractions.
For example, in Rubik's Cube one could choose the reference locations to
be two diagonally opposite corner locations.
Note that each operator only changes one of these locations.
An abstract state transition would have a primary cost of 1 if the cubie
it moved into one of these locations was a distinguished cubie in its
abstraction, and a primary cost of 0 otherwise.

Although the cost-splitting and location-based methods for defining
costs can be applied to a wide range of state spaces, they are not
guaranteed to define heuristics that are superior to other
heuristics for a given state space. We determined experimentally
that heuristics based on cost-splitting substantially improve
performance for sufficiently large versions of TopSpin and that
heuristics based on location-based costs vastly improve the state of
the art for the 17-Pancake puzzle. In our experiments additive
heuristics did not improve the state of the art for Rubik's Cube.
The following subsections describe the positive results in detail.
The negative results are discussed in Section \ref{negative}.






